Distributed LSTM-Learning from Differentially Private Label Proportions

Data privacy and decentralised data collection has become more and more popular in recent years. In order to solve issues with privacy, communication bandwidth and learning from spatio-temporal data, we will propose two efficient models which use Differential Privacy and decentralized LSTM-Learning: One, in which a Long Short Term Memory (LSTM) model is learned for extracting local temporal node constraints and feeding them into a Dense-Layer (LabelProportionToLocal). The other approach extends the first one by fetching histogram data from the neighbors and joining the information with the LSTM output (LabelProportionToDense). For evaluation two popular datasets are used: Pems-Bay and METR-LA. Additionally, we provide an own dataset, which is based on LuST. The evaluation will show the tradeoff between performance and data privacy.

==> graphics/histogramTransfer.tex <==


\begin{figure*}[]
    \centering
    \begin{tikzpicture}[scale=4]
	\draw[] (-1.2,0) rectangle +(0.1,0.1) node[pos=.5] {$x_l$};
	\draw[] (-1.1,0) rectangle +(0.1,0.1) node[pos=.5] {1};
	\draw[] (-1,0) rectangle +(0.1,0.1) node[pos=.5] {0};
	\draw[] (-0.9,0) rectangle +(0.1,0.1) node[pos=.5] {1};
	\draw[] (-0.8,0) rectangle +(0.1,0.1) node[pos=.5] {1};
	\draw[] (-0.7,0) rectangle +(0.1,0.1) node[pos=.5] {2};
	\draw[] (-0.6,0) rectangle +(0.1,0.1) node[pos=.5] {0};
	
	\node (measurementText) at (-0.85,-0.06) {measurement values};
	
	\draw[->] (-0.4,0.05) -- (-0.25,0.05);

	\draw[fill,lightgray] (-0.2,0) rectangle +(0.1,0.2);
	\node (label0) at (-0.15,-0.06) {0};
    \draw[fill,gray] (-0.1,0) rectangle +(0.1,0.3);
    \node (label1) at (-0.05,-0.06) {1};
    \draw[fill,black] (0.0,0) rectangle +(0.1,0.1);
    \node (label2) at (0.05,-0.06) {2};
    
    \draw[->] (0.15,0.05) -- (0.45,0.05) node[midway,above] {noise};
    
    
    \draw[fill,lightgray] (0.5,0) rectangle +(0.1,0.2);
    \draw[black] (0.5,0.2) rectangle +(0.1,0.02);
	\node (label0) at (0.55,-0.06) {0};
    \draw[fill,gray] (0.6,0) rectangle +(0.1,0.3);
    \draw[black] (0.6,0.3) rectangle +(0.1,0.01);
    \node (label1) at (0.65,-0.06) {1};
    \draw[fill,black] (0.7,0) rectangle +(0.1,0.1);
    \draw[black] (0.7,0.1) rectangle +(0.1,0.03);
    \node (label2) at (0.75,-0.06) {2};
    
    \draw[->] (0.9,0.05) -- (1.8,0.05) node[midway,text width=2cm,align=center] {transfer to neighbor};
    
    \draw[dashed,rounded corners] (2.2,-0.2) -- (1.7,-0.2) -- (1.7,0.4) -- (2.2,0.4);
    \draw[dashed,rounded corners] (-1.4,-0.2) -- (1.6,-0.2) -- (1.6,0.4) -- (-1.4,0.4);
    \node (labelJ) at (1.9,0.3) {$j$};
    \node (labelNeighbor) at (-0.85,0.3) {$n_i(j)$};
\end{tikzpicture}
    \caption{Example for data exchange. Original measurement values from $n_i(j)$ are used to build up a histogram, to which noise is added. Noise is shown in the second histogram by the white boxes with black border. Resulting histograms are send to the node $j$, that is currently learning the model.}
    \label{fig:histogramTransfer}
\end{figure*}
